Hausdorff and box dimension bounds for subfractals induced by $S$-gap shifts

In this paper, we consider subsets of an attractor of an iterated function system in which each point is associated with an allowable word from an $S$-gap shift. The main result shows that bounds for the box dimension and Hausdorff dimension of a subfractal induced by an $S$-gap shift are given by the zeros of the upper and lower topological pressure functions.

==> sgapbib.tex <==
@article {Deliuetal,
    AUTHOR = {Deliu, Anca and Geronimo, J. S. and Shonkwiler, R. and Hardin,
              D.},
     TITLE = {Dimensions associated with recurrent self-similar sets},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {110},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {327--336},
      ISSN = {0305-0041},
   MRCLASS = {58F11 (26A18 28A80)},
  MRNUMBER = {1113431},
MRREVIEWER = {Tim Bedford},
       DOI = {10.1017/S0305004100070407},
       URL = {http://dx.doi.org/10.1017/S0305004100070407},
}

@incollection {EllisBranton,
    AUTHOR = {Ellis, David B. and Branton, Michael G.},
     TITLE = {Non-self-similar attractors of hyperbolic iterated function
              systems},
 BOOKTITLE = {Dynamical systems ({C}ollege {P}ark, {MD}, 1986--87)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1342},
     PAGES = {158--171},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1988},
   MRCLASS = {58F12},
  MRNUMBER = {970553},
MRREVIEWER = {Nima Geffen},
       DOI = {10.1007/BFb0082829},
       URL = {http://dx.doi.org/10.1007/BFb0082829},
}

@book {FalconerFG,
    AUTHOR = {Falconer, Kenneth},
     TITLE = {Fractal geometry},
   EDITION = {Third},
      NOTE = {Mathematical foundations and applications},
 PUBLISHER = {John Wiley \& Sons, Ltd., Chichester},
      YEAR = {2014},
     PAGES = {xxx+368},
      ISBN = {978-1-119-94239-9},
   MRCLASS = {28-01 (11K55 28A78 28A80 37C45 37F10)},
  MRNUMBER = {3236784},
MRREVIEWER = {Manuel Mor\'an},
}

@book {FalconerTech,
    AUTHOR = {Falconer, Kenneth},
     TITLE = {Techniques in fractal geometry},
 PUBLISHER = {John Wiley \& Sons, Ltd., Chichester},
      YEAR = {1997},
     PAGES = {xviii+256},
      ISBN = {0-471-95724-0},
   MRCLASS = {28A80 (00A69 11K55 58F13)},
  MRNUMBER = {1449135},
MRREVIEWER = {Christoph Bandt},
}

@article {Hutchinson,
    AUTHOR = {Hutchinson, John E.},
     TITLE = {Fractals and self-similarity},
   JOURNAL = {Indiana Univ. Math. J.},
  FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {30},
      YEAR = {1981},
    NUMBER = {5},
     PAGES = {713--747},
      ISSN = {0022-2518},
   MRCLASS = {49F20 (00A69 28A12 58C27)},
  MRNUMBER = {625600},
MRREVIEWER = {F. J. Almgren, Jr.},
       DOI = {10.1512/iumj.1981.30.30055},
       URL = {http://dx.doi.org/10.1512/iumj.1981.30.30055},
}

@book {LindMarcus,
    AUTHOR = {Lind, Douglas and Marcus, Brian},
     TITLE = {An introduction to symbolic dynamics and coding},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1995},
     PAGES = {xvi+495},
      ISBN = {0-521-55124-2; 0-521-55900-6},
   MRCLASS = {58F03 (15A48 54H20 58F20 94A24 94B60)},
  MRNUMBER = {1369092},
MRREVIEWER = {Petr K rka},
       DOI = {10.1017/CBO9780511626302},
       URL = {http://dx.doi.org/10.1017/CBO9780511626302},
}



@article {Roychowdhury,
    AUTHOR = {Roychowdhury, Mrinal Kanti},
     TITLE = {Hausdorff and upper box dimension estimate of hyperbolic
              recurrent sets},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {201},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {507--523},
      ISSN = {0021-2172},
   MRCLASS = {28A78},
  MRNUMBER = {3265293},
MRREVIEWER = {Ezequiel Rela},
       DOI = {10.1007/s11856-014-0028-0},
       URL = {http://dx.doi.org/10.1007/s11856-014-0028-0},
}


@article{DastjerdiSgap, 
author={Dawoud Ahmadi Dastjerdi and Somaye Jangjoo},
title={Dynamics and Topology of S-gap Shifts},
journal={Topology and its Applications},
volume={159},
year={2012},
pages={2654-2661}
}

@article {CT,
    AUTHOR = {Climenhaga, Vaughn and Thompson, Daniel},
     TITLE = {Intrinsic ergodicity beyond specification: $\beta$-shifts, $S$-gap shifts, and their factors},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {192},
      YEAR = {2012},
    NUMBER = {2},
     PAGES = {785–817},
}

@book {Walters,
    AUTHOR = {Walters, Peter},
     TITLE = {An introduction to ergodic theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {79},
 PUBLISHER = {Springer-Verlag, New York-Berlin},
      YEAR = {1982},
     PAGES = {ix+250},
      ISBN = {0-387-90599-5},
   MRCLASS = {28Dxx (54H20 58F11)},
  MRNUMBER = {648108},
MRREVIEWER = {M. A. Akcoglu},
}




@article {Sattler,
    AUTHOR = {Sattler, Elizabeth},
     TITLE = {Fractal dimensions of subfractals induced by sofic subshifts},
   JOURNAL = {Monatsh. Math.},
  FJOURNAL = {Monatshefte f\"ur Mathematik},
    VOLUME = {183},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {539--557},
}

@article {Spandl,
    AUTHOR = {Spandl, Christoph},
     TITLE = {Computing the topological entropy of shifts},
   JOURNAL = {MLQ Math. Log. Q.},
  FJOURNAL = {MLQ. Mathematical Logic Quarterly},
    VOLUME = {53},
      YEAR = {2007},
    NUMBER = {4-5},
     PAGES = {493-510},
}


